MemEye: A Visual-Centric Evaluation Framework for Multimodal Agent Memory

Long-term agent memory is increasingly multimodal, yet existing evaluations rarely test whether agents preserve the visual evidence needed for later reasoning. In prior work, many visually grounded questions can be answered using only captions or textual traces, allowing answers to be inferred without preserving the fine-grained visual evidence. Meanwhile, harder cases that require reasoning over changing visual states are largely absent. Therefore, we introduce MemEye, a framework that evaluates memory capabilities from two dimensions: one measures the granularity of decisive visual evidence (from scene-level to pixel-level evidence), and the other measures how retrieved evidence must be used (from single evidence to evolutionary synthesis). Under this framework, we construct a new benchmark across 8 life-scenario tasks, with ablation-driven validation gates for assessing answerability, shortcut resistance, visual necessity, and reasoning structure. By evaluating 13 memory methods across 4 VLM backbones, we show that current architectures still struggle to preserve fine-grained visual details and reason about state changes over time. Our findings show that long-term multimodal memory depends on evidence routing, temporal tracking, and detail extraction.

==> Section/section3.tex <==
\section{The Taxonomy of \sys}

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{Fig/xyaxis.pdf}
  \caption{Taxonomy and distribution of the MemEye dataset across domains and tasks. The inner ring groups tasks by life-scenario domain; the outer ring shows individual tasks with their question counts.}
  \label{fig:xyaxis}
\end{figure}

In \sys, we introduce an understanding centric benchmark that constructs a two dimensional evaluation space along two orthogonal axes (illustrated in~\autoref{fig:xyaxis}. Each axis captures a distinct but complementary capability required for robust agent performance. The X-axis measures the granularity of decisive visual evidence that must be preserved and interpreted: $X_1$ scene-level evidence, $X_2$ region-level evidence, $X_3$ instance-level evidence, and $X_4$ pixel-level evidence. In our benchmark, answering a question is grounded in genuine image understanding rather than relying on surface-level cues such as captions. After retrieving the relevant image, the agent must interpret information across this hierarchy, from scene-level context to pixel-level details, in order to produce a correct answer.  The $Y$-axis evaluates the agent’s ability to locate sufficient and reliable evidence for answering the question, emphasizing not only retrieval accuracy but also the completeness of supporting information.  Together, the two axes disentangle \emph{what visual evidence must be extracted} from \emph{how that evidence is used over memory}.

Here is the detailed definition of the coordinates:

\paragraph{$X_1$: Scene-level}
$X_1$ measures whether the model preserves scene-level evidence, focusing on the overall scene type, activity, and global semantic gist of an image. This level is largely caption-recoverable and thus serves as the coarsest visual baseline and a lower bound in Caption-Proof analysis.
\paragraph{$X_2$: Region-level}
$X_2$ evaluates the ability to perceive and reason over semantically coherent regions within a scene. The model must identify meaningful subregions (e.g., functional areas or grouped entities) and capture their local context and interactions. Unlike scene-level understanding, this level focuses on region-level semantics, where information is organized within localized areas rather than across the entire scene. Caption-only representations often collapse such regional structures into coarse descriptions, making this a critical boundary for region-aware visual understanding.
\paragraph{$X_3$: Instance-level}
$X_3$ evaluates whether the model can localize and distinguish specific object or person instances within and across images. The key challenge is no longer understanding a region as a coherent local scene, but preserving which concrete entity is being referred to (e.g., “the earlier mug”) when multiple visually or semantically similar candidates exist. Caption-based representations often flatten these instance-level distinctions, marking the transition from region-level understanding to instance-level visual memory.
\paragraph{$X_4$: Pixel-level}
$X_4$ requires reasoning over pixel-level evidence expressed through fine-grained visual details (e.g., subtle color, texture, small text). These cues are often omitted in text, capturing what we term intra-pixel necessity—where critical evidence exists only in the visual signal.
\paragraph{$Y_1$: Atomic Retrieval}
$Y_1$ measures whether the model can retrieve a single fact from memory without cross-session reasoning. It primarily tests basic memory access rather than composition, serving as the lowest reasoning baseline.
\paragraph{$Y_2$: Relational Association}
$Y_2$ evaluates the ability to associate distributed evidence across sessions, modalities, or references. The reasoning remains monotonic: information accumulates without contradiction. This level captures referential resolution and implicit memory traversal beyond isolated retrieval.
\paragraph{$Y_3$: Evolutionary Synthesis}
$Y_3$ tests non-monotonic synthesis over evolving memory. The model must handle updates, conflicts, and overrides, maintaining a coherent world state under revision. Answers are not explicitly stated but must be inferred from changing evidence.

